Empirical evaluation of Uncertainty Quantification in Retrieval-Augmented Language Models for Science

Large language models (LLMs) have shown remarkable achievements in natural language processing tasks, producing high-quality outputs. However, LLMs still exhibit limitations, including the generation of factually incorrect information. In safety-critical applications, it is important to assess the confidence of LLM-generated content to make informed decisions. Retrieval Augmented Language Models (RALMs) is relatively a new area of research in NLP. RALMs offer potential benefits for scientific NLP tasks, as retrieved documents, can serve as evidence to support model-generated content. This inclusion of evidence enhances trustworthiness, as users can verify and explore the retrieved documents to validate model outputs. Quantifying uncertainty in RALM generations further improves trustworthiness, with retrieved text and confidence scores contributing to a comprehensive and reliable model for scientific applications. However, there is limited to no research on UQ for RALMs, particularly in scientific contexts. This study aims to address this gap by conducting a comprehensive evaluation of UQ in RALMs, focusing on scientific tasks. This research investigates how uncertainty scores vary when scientific knowledge is incorporated as pretraining and retrieval data and explores the relationship between uncertainty scores and the accuracy of model-generated outputs. We observe that an existing RALM finetuned with scientific knowledge as the retrieval data tends to be more confident in generating predictions compared to the model pretrained only with scientific knowledge. We also found that RALMs are overconfident in their predictions, making inaccurate predictions more confidently than accurate ones. Scientific knowledge provided either as pretraining or retrieval corpus does not help alleviate this issue. We released our code, data and dashboards at https://github.com/pnnl/EXPERT2.

==> sections/background.tex <==
\section{Background}

\cite{xiao2022uncertainty} mentions different quantifiers for uncertainty. Temperature Scaling is one such technique that is used to quantify uncertainty in machine learning model predictions by providing a measure of how confident the model is in its predictions. A higher temperature indicates that the model is less confident in its prediction. To quantify uncertainty using temperature scaling, we can calculate the entropy of the model's output distribution using temperature-scaled logits. Entropy is a measure of the uncertainty of a probability distribution. A higher entropy indicates a more uncertain distribution \citep{guo2017calibration}

% \anurag{Following portions of this section reads more like a related works section. We should move some of these parts to the next section, or else reword it to be more introductory.}

Monte Carlo (MC) Dropout is another technique that can be used to estimate the uncertainty of machine learning model predictions. It works by averaging the results of multiple forward passes through the model with dropout turned on. Dropout is a regularization technique that randomly deactivates a certain percentage of neurons in the model during training, helping the model from overfitting. MC Dropout is a powerful tool for estimating the uncertainty of machine learning model predictions. It is simple to implement and can be used with a variety of different model architectures \citep{gal2016dropout}\

Other uncertainty quantifiers include Ensemble and LL SVI (Last-Layer Stochastic Variational Inference). Ensemble learning works by combining the predictions of multiple independently trained models \citep{lakshminarayanan2017simple}, while LL SVI uses variational inference to approximate the posterior predictive distribution of the model \citep{blundell2015weight}. Both techniques can be effective for improving the reliability and robustness of machine learning models.

% \textcolor{red}{briefly what experiments we did}
In our current work, we experiment with different uncertainty measure to assess the reliability of RALM using three benchmark datasets. We intend to find how uncertainty scores vary when scientific knowledge is added as the pretraining data and further explore the variation of uncertainty scores with the accuracy of the predicted outputs. These experiments are conducted across two RALMs - one with scientific knowledge is added as the pretraining data and the other with general knowledge added as the pretraining data. 

% Uncertainty quantification is 
% Retrieval Augmented Language Model (RALM) is a framework that augments language model pre-training algorithms by incorporating a learned textual knowledge retriever.\citep{guu2020retrieval}.
% RALM is well known for improving the quality of Large Language Models (LLMs)by grounding them on external sources of knowledge. REALM offers advantages like
% \begin{itemize}
%     \item Improved accuracy:  since they are better able to access and process factual information, which makes them more accurate on tasks such as question answering and summarizing  
%     \item Deceased hallucinations: Less likely to generate factually incorrect information since they rely on external knowledge. 
%     \item Increased transparency: Provides evidences by linking the relevant documents retrieved from the knowledge corpus. 
% \end{itemize}
% what's UQ in generative language model, standard procedure to compute UQ
% Several research studies have been conducted in the area of uncertainty quantification for LLMs to assess the reliability of their responses. However little to no research has been conducted in the area of uncertainty quantification for RALM. In our work, we have performed several experiments to evaluate the behavior of uncertainty quantification on REALM, thus pioneering the quantification of uncertainty for RALM.
% Summerize our UQ work in 4- 5 sentences. 


==> sections/limitations.tex <==
\paragraph{\textbf{Limitations}}
All our experiments are based on ATLAS base size, i.e., $220M$. In the future, we will conduct experiments on larger scale models to analyze the impact of scale on UQ measures. In addition, we compare ATLAS model pretrained from scratch on scientific literature corpus with that of pretrained with general domain CC/Wiki corpus. It will be interesting to incorporate results from model that is adapted from general domain by continual pretraining on scientific corpus.
